Proximal Causal Learning with Kernels: Two-Stage Estimation and Moment Restriction

We address the problem of causal effect estimation in the presence of unobserved confounding, but where proxies for the latent confounder(s) are observed. We propose two kernel-based methods for nonlinear causal effect estimation in this setting: (a) a two-stage regression approach, and (b) a maximum moment restriction approach. We focus on the proximal causal learning setting, but our methods can be used to solve a wider class of inverse problems characterised by a Fredholm integral equation. In particular, we provide a unifying view of two-stage and moment restriction approaches for solving this problem in a nonlinear setting. We provide consistency guarantees for each algorithm, and we demonstrate these approaches achieve competitive results on synthetic data and data simulating a real-world task. In particular, our approach outperforms earlier methods that are not suited to leveraging proxy variables.

==> connection.tex <==

%%%
\subsection{Connection Between the Two Approaches}
\label{sec:connection}



\begin{remark}
We note a key difference between the closed form solutions of KPV and PMMR. In KPV, the
\end{remark}



\textcolor{red}{\textbf{Contrast and connection with the KPV formulation.} Note that under the KPV formulation, we obtained that $h$ is a linear combination of outer products of \textit{all} combinations of feature maps $(\{k(a_i,\cdot)\}_{i=1}^n, \{k(x_i,\cdot)\}_{i=1}^n)$, and $\{k(w_j,\cdot)\}_{j=1}^n$, i.e.
\begin{equation}
        h^{KPV}(a,w,x) = \sum_{i,j=1}^n \hat{h}^{KPV}_{ij} k(a_i,a)k(x_i,x)k(w_j,w)
\end{equation}
\textbf{Why do we get two different representations of $h$?} 
At their roots, the KPV and MMR approaches minimises different risk functionals  (c.f. \Cref{sec:connection}). KPV aims to minimise  $\mathbb{E}_{A,Z,Y,X}[\|Y - \mathbb{E}[h(A,W,X)|A,Z,X]\|^2]$ over $h$. In particular, for every sample $(a_i,z_i,y_i,w_i, x_i)$, $\mathbb{E}_{W}[h(a_i,W,x_i)|a_i,z_i,x_i]$ needs to be computed, which in turn requires the the feature maps at $a_i$ and $x_i$ and those at \textit{all} \(\{w_i\}_{i=1}^n\) in order to compute the conditional mean embedding $\mu_{W|a_i,z_i,x_i}$. Meanwhile, MMR minimises \(\mathbb{E}[(Y- h(A,W,X))(Y' - h(A',W',X'))k((A,Z,X), (A',Z',X'))]\label{eq:r_k}\), where the expression inside the expectation operator is not a function of \(\mathbb{E}[h|A,W,X]\). This means that, for every sample $\{a_i, z_i,y_i,w_i,x_i\}$, we only need to compute $h(a_i,w_i,x_i)$, which only requires the features at $a_i$, $x_i$ and $w_i$. To make this concrete, we formally check the application of the representer theorem in the Appendix (\ref{apprendix: representer_MMR}). }



Several authors have made an insightful relationship between the negative controls and nonparametric IV (NPIV) regression \citep{miao2018confounding,miao2018identifying,deaner2021proxy,tchetgen2020introduction}, especially in solving \eqref{eq:integral-eq} using tools developed in the NPIV literature \citep{Ai03:CMR,Newey03:NPIV}. 
The 2SLS and GMM \citep{Angrist08:Harmless, Hansen82:GMM} are the most well-known approaches that have recently gained popularity in the ML community \citep{Hartford17:DIV,Bennett19:DeepGMM,Muandet19:DualIV,Dikkala20:Minimax,zhang2020maximum}.
While the connection between 2SLS and GMM estimators were established in the linear setting, similar connection in a nonlinear setting remains an open question.
This section elucidates the connection between our KPV and PMMR algorithms through the len of NPIV setting.

%Let us assume a structural equation with additive noise model
%$Y = f(X) + \varepsilon$
%where $f$ is an unknown, potentially non-linear continuous function.
%We assume that the additive noise $\varepsilon$ has zero mean, i.e., $\mathbb{E}[\varepsilon] = 0$ and is correlated with the input $X$, i.e., $\mathbb{E}[\varepsilon\,|\,X] \neq 0$. 
%Let $Z$ be an instrumental variable such that $\mathbb{E}[\varepsilon\,|\,Z] = 0$. 
%that satisfies the following three assumptions: (i) \emph{relevance}: $Z$ has causal influence on $X$, (ii) \emph{exclusion restriction}: $Z$ has no direct effect on $Y$, i.e., $Y \perp \!\!\! \perp Z\,|\,X,\varepsilon$, and (iii) \emph{exchangeability}: $Z$ does not share common causes with the outcome $Y$, i.e., $Z \perp \!\!\! \perp \varepsilon$.
In the NPIV, we aim to solve the Fredholm integral equation of the first kind:
\begin{equation}\label{eq:fredholm}
    \mathbb{E}[Y\,|\,z] = \int_{\mathcal{X}} f(X) \,dP(X|z), \quad \forall z\in\mathcal{Z},
\end{equation}
where, with an abuse of notation, $X$, $Y$, and $Z$ denote endogeneous, outcome, and instrumental variables, respectively.
Solving \eqref{eq:fredholm} for $f$ is known to be an ill-posed inverse problem in a nonparametric setting \citep{Carrasco07:LIP}.

\vspace{-7pt}
\paragraph{Two-stage approach.}

Like DeepIV \citep{Hartford17:DIV} and KernelIV \citep{singh2019kernel}, the KPV algorithm is a two-stage approach.
In the first stage, an estimate of the integral on the rhs of \eqref{eq:fredholm} is constructed. In the second stage, the function $f$ is then learned to minimize the discrepancy between the lhs and the estimated rhs of \eqref{eq:fredholm}. 
Formally, this can be formulated via the unregularized risk functional
\begin{eqnarray}
    R(f) &:=& \mathbb{E}_{Z}[(\mathbb{E}[Y|Z] - \mathbb{E}[X\,|\,Z])^2] \label{eq:natural-loss}\\
        &\leq& \mathbb{E}_{\mathit{YZ}}[(Y - \mathbb{E}[f(X)\,|\,Z])^2] =: \tilde{R}(f). \label{eq:surrogate-loss}
\end{eqnarray}
This risk functional \eqref{eq:surrogate-loss} is considered in DeepIV \cite{Hartford17:DIV}, KernelIV \cite{singh2019kernel}, and DualIV \cite{Muandet19:DualIV}. 
Both DeepIV and KernelIV (including our KPV) directly solve the surrogate loss \eqref{eq:surrogate-loss}, whereas DualIV solves the dual form of \eqref{eq:surrogate-loss}.

%By the law of total expectation, we can bound the risk functional \eqref{eq:two-stage-loss} from above by
%\begin{eqnarray*}
%    \mathbb{E}_{\mathit{YZ}}[(Y - \mathbb{E}[f(X)\,|\,Z])^2]
%    &=& \mathbb{E}_{Z}[\mathbb{E}_{Y|Z}[(Y - \mathbb{E}[f(X)\,|\,Z])^2\,|\,Z]] \\
%    &\geq& \mathbb{E}_{Z}[(\mathbb{E}_{Y|Z}[Y - \mathbb{E}[f(X)\,|\,Z] \,|\,Z])^2] \\
%    &=& \mathbb{E}_{Z}[(\mathbb{E}[Y|Z] - \mathbb{E}[f(X)\,|\,Z])^2] \\
%    &=:& \tilde{R}(f).
%\end{eqnarray*}

The natural risk functional \eqref{eq:natural-loss} is also considered in \citet{Liao20:NeuralSEM}, which shows that there is a connection between this risk functional and the classical GMM objective; see \citet[Appendix F]{Liao20:NeuralSEM}.
Unlike \citet{Liao20:NeuralSEM}, we unravel a deeper connection between modern two-stage procedures and the GMM-based counterparts.

\vspace{-7pt}
\paragraph{GMM-based approach.}

Instead of \eqref{eq:fredholm}, an alternative starting point to NPIV is a conditional moment restriction (CMR) $\mathbb{E}[\varepsilon\,|\,Z] = \mathbb{E}[Y - f(X)\,|\,Z] = 0$ \citep{miao2018confounding,deaner2021proxy,Dikkala20:Minimax,zhang2020maximum}.
This CMR implies that
\begin{equation}\label{eq:unconditional_MR}
    \mathbb{E}_{\mathit{XYZ}}[(Y - f(X))h(Z)] = 0
\end{equation}
for any measurable function $h$.
This follows from the law of iterated expectation: $\mathbb{E}_{\mathit{XYZ}}[(Y - f(X))h(Z)] =  \mathbb{E}_{\mathit{XY}}[\mathbb{E}_Z[(Y - f(X))h(Z)\,|\,Z]] = \mathbb{E}_{\mathit{XY}}[\mathbb{E}_Z[(Y - f(X))\,|\,Z]h(Z)]$.
In \citet{Bennett19:DeepGMM} and \citet{Dikkala20:Minimax}, the function $f$ can be obtained as a solution to the following unregularized minimax optimization problem:
\begin{equation}\label{eq:minimax}
    \min_{f\in L_2(X)}\max_{h\in L_2(Z)}\; \mathbb{E}_{\mathit{XYZ}}[(Y - f(X))h(Z)]. 
\end{equation}
In a similar line of work, \citet{Muandet20:KCM} shows that a reproducing kernel Hilbert space (RKHS) for $h$ is sufficient in the sense that the inner maximum moment restriction (MMR) preserves all information about the original CMR.
In \citet{zhang2020maximum}, the MMR is used for the IV regression problem.

\vspace{-7pt}
\paragraph{The connection.}

Following \citet[Sec 3.2]{Muandet19:DualIV}, if we apply the interchangeability principle and Fenchel duality to $R(f)$, we obtain the following dual formulation\footnote{The same result appears in \citet[Appendix F]{Liao20:NeuralSEM}.}
\begin{equation*}
    \min_{f\in L_2(X)}\max_{h\in L_2(Z)}\; \mathbb{E}_{\mathit{XYZ}}[(Y - f(X))h(Z) - \frac{1}{2}h^2(Z)],
\end{equation*}
which is equivalent to \eqref{eq:minimax} up to the second term $\mathbb{E}_{\mathit{XYZ}}[\frac{1}{2}h^2(Z)]$.
Applying the same derivation to $\tilde{R}(f)$ gives
\begin{equation*}
    \min_{f\in L_2(X)}\max_{h\in L_2(Y,Z)}\; \mathbb{E}_{\mathit{XYZ}}[(Y - f(X))h(Y,Z) - \frac{1}{2}h^2(Y,Z)],
\end{equation*}
which is the objective function of DualIV \citep{Muandet19:DualIV}. 
In other words, DeepIV \citep{Hartford17:DIV} and KernelIV \citep{singh2019kernel} (resp. KPV) solve an objective function that is an upper bound of the problem whose dual form coincides with the adversarial objective used in AdversarialGMM \citep{Dikkala20:Minimax}, DeepGMM \citep{Bennett19:DeepGMM}, and MMR-IV \citep{zhang2020maximum} (resp. PMMR). 
Moreover, DualIV solves an objective that differs from the GMM-based approaches because $h(Y,Z)$ violates the exclusion restriction and cannot be interpreted as an instrument.
These observations reveal the close connection between modern nonlinear methods for NPIV, as well as between our KPV and PMMR algorithms.


\begin{thm}\label{th:connection}
    %Under which conditions the solutions coincide?
    %\begin{equation}
      %  f^* = \arg\min_{f\in\mathcal{F}}\, R(f) = \arg\min_{f\in\mathcal{F}}\, \tilde{R}(f).
    %\end{equation}
    Assume there exists $f^* \in L^2_{P_X}$ such that $\E[Y|Z]=\E[f^*(X)|Z]$.
    \begin{enumerate*}[label=(\roman*)]
        \item $f^*$ is a minimizer of $R$ and $\tilde{R}$.
        \item Assume $k$ satisfies \Cref{ass:ispd}. Then $R_k(f) \eqdef \sup_{h\in \Hx}\E_{XYZ}[(Y-f(X))h(Z)] = 0$ iff $R(f)=0$.
        \item \citet[Theorem 1]{Muandet20:KCM}. Assume $k$ satisfies \Cref{ass:kernel_characteristic}. Assume $f^* \in \cH_{X}$ and that %the conditional mean embedding operator of $P_{X|Z}$ is Hilbert-Schmidt. 
        $\E[f(X)|Z=\cdot]\in \Hz$.
        Then, $f^*$ is given by the Kernel Instrumental Variable Approach (or kernel 2SLS), and is a minimizer of $R$ and $\tilde{R}$. 
        \end{enumerate*}
\end{thm}

See \Cref{sec:connection_proof} for the proof of \Cref{th:connection}. %Result 2 corresponds to \citet[Theorem 1]{Muandet20:KCM}. %Notice the minimizers of $R$ and $\tilde{R}$ may not unique in general.  
Under \Cref{ass:kernel_characteristic} and $\E[f(X)|Z]\in \Hz$, the conditional mean embedding of $P_{X|Z}$ (equivalently, the conditional mean embedding operator) characterizes the full distribution $P_{X|Z}$. %It replaces the completeness condition which states that the conditional expectation of $X|Z$ is injective. \ak{double check the statement and proof please :)}


==> private.tex <==
\subsection{Warm-up \textcolor{red}{updated 31.12.20}}
\textbf{Structural Equations.} For simplicity, we assume $X$ is null, and the structural equations we use are listed as follows:
\begin{eqnarray}
U &\sim& \chi^2(5)\\
Z &=& - U - 1 + \mathcal{N}(0, 1)\\
W &=& 2U + 2 +\mathcal{N}(0, 1)\\
A &=& 2\sqrt{U} + \mathcal{N}(0,1)\\
Y &=& A\sin(0.5A) - \log_{10}(U) + \mathcal{N}(0, 1)\\
\end{eqnarray}
\begin{eqnarray}\label{eq:structural1}
U &\sim& Unif[1,10]\\
Z &=& - U - 1 + \mathcal{N}(0, 1)\\
W &=& 2U + 2 +\mathcal{N}(0, 1)\\
A &=&(2U + \mathcal{N}(0,1))\sin(2U + \mathcal{N}(0,1)) + 10\\
Y &=& 0.5A\sin(0.5A) + 2U + \mathcal{N}(0, 1)\\
\end{eqnarray}
\textcolor{red}{update 31.12.20: only the eq for A changed.}
\begin{figure}[h!]
\includegraphics[scale=0.4]{plots/MMR_plots/asinaMildNonlinearA/full_pairwise.png}
\caption{Here we show the scatter of data generated from the above structure equations (courtesy to Afsaneh's nice seaborn routine).}
\end{figure}
\begin{figure}[h!]

\centering
\includegraphics[scale=0.6]{plots/MMR_plots/asinaMildNonlinearA/ate_pairwise.png}
    \caption{And here is the ATE plot.}
\end{figure}
\subsection{Full Proxy Graph \textcolor{red}{update 31.12.20: again only the eq for A changed.}}
Now that we have shown the efficacy of our methods on the simplified causal graph, we transition to the full proxy graph as in Figure \ref{fig:causal_diagram}, again omitting $x$. 
\textbf{Structural Equations.} We again list the structural equations of the full graph here.
\begin{eqnarray}\label{eq:structural2}
U &\sim& Unif[1,10]\\
Z &=& - U - 1 + \mathcal{N}(0, 1)\\
W &=& 2U + 2 +\mathcal{N}(0, 1)\\
A &=& (2U + 0.5Z + \mathcal{N}(0,1))\sin(2U + 0.5Z + \mathcal{N}(0,1)) + 10\\
Y &=& 0.5A\sin(0.5A) + 2U + 0.5W + \mathcal{N}(0, 1)\\
\end{eqnarray}
\textcolor{red}{update 31.12.20: again only the eq for A changed.}

\section{Conditional metric generation}
\begin{figure}[h!]
\includegraphics[scale=0.4]{plots/MMR_plots/rbfNonLinearYFullTrain10000scaledSig2/full_pairwise.png}
\caption{Here we show the scatter of data generated from the above structure equations.}\label{fig:full_rbfNonLinearYFull}
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[scale=0.6]{plots/MMR_plots/rbfNonLinearYFullTrain10000scaledSig2/ate_pairwise.png}
\caption{And here is the ATE plot.} \label{fig:ate_rbfNonLinearYFull}
\end{figure}

\subsection{Evaluation Metrics}
We would like one of our evaluation metrics to be:
\begin{equation}
    \mathcal{L}(a,x,z) = |\mathbb{E}[Y - h(a,x,w)|a,x,z]|
\end{equation}

which we may approximate as:

\begin{equation}
    \hat{\mathcal{L}}(a,x,z) = \left |\frac{1}{N}\sum_{i=1}^N y_i(a,x,z) - h(a,x,w_i(a,x,z))\right |
\end{equation}

where $y_i(a,x,z)$ and $w_i(a,x,z)$ denotes the $i^{th}$ sample of $Y$ and $W$, respectively, when $A, X, Z$ take values $a, x, z$. 

Empirically, we use the simulation to generate values for the entire domains for all variables $(A,X,W,Z,Y)$, then take the slice for fixed values of $(A,X,Z)$. The pseudocode is given below:

\begin{algorithm}[H]
\SetAlgoLined
\KwResult{A,X,Z, Wsamples, avYgivenAXZ }
Sample triples (a,x,z) at random, within the range of the realistic domains of A, X, Z. \;
Sample Tuples = M tuples (a,x,z,w,y) from simulation. \;
Shuffle the columns of Tuples. \;
Select threshold for minimum valid samples for Y and W. \;

 \For{each triple (a,x,z)}{
  Select the subset of M tuples sufficiently close to (a,x,z). Output = subTuples.\;
  \eIf{number of columns in subTuples $<$ thresh}{
   break. \;
   }{
   subTuples = subTuples[:, :thresh]\;
  }
  Take the average for the Y values in subTuple. Append to avYgivenAXZ. \;
  Save the samples of W in subTuple. Append to Wsamples.\;
 }
 \caption{Generating evaluation samples}
\end{algorithm}

% sample triples (a,x,z) at random, within the range of the realistic domains of A, X, Z. shape: 3 x N_3.

% sample Tuples = M tuples (a,x,z,w,y) from simulation, shuffle. shape: 5 x N_5.

% select threshold for minimum valid samples for Y and W. Out: thresh

% axz, y, w_samples = [], [], []

% for each triple (a,x,z):
%       1. select the subset of M tuples sufficiently            close to (a,x,z). Out: sub_Tuples
%       2. if sub_Tuples.shape[-1] < thresh: break;             else: sub_Tuples = sub_Tuples[:, :thresh]
%       3. take the average of Y|a,x,z. Out: Yaxz_av
%       4. axz.append((a,x,z)), y.append(Yaxz_av),              w_samples.append(sub_Tuples[-2,:]). 

% axz_np = np.array(axz)
% y_np = np.array(y)
% axzy_np = np.concatenate([axz_np, y_np.reshape(-1,1))
% w_samples_np = np.array(w_samples)
% np.savez(fpath, axzy=axzy_np, w_samples=w_samples_np)

% To derive closed form RKHS solution from MMR_for_IVR code base:
% first load params from file
% then compute alpha from params
% then compute test_L0 from causal effect test data one by one.
% for each a in do_A, repeat itself the same number of times as w and concatenate with w.
% compute test_L0 by taking the square distance with training data. 
% compute test_L using test_L0.
% compute prediction with pred = test_L @ alpha for the whole vector of aw.
% get causal effect by averaging the aw.


\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
       Models.        & MMR-rkhs& DirectNN & NN2SLS & Vanilla2SLS & Poly2SLS & AdjustNN & GMM\\
       \hline
       Causal MAE     & 0.103   & 0.287    & 0.905  & 0.148       & 1.123    & 0.280    & 0.239\\
       \hline
       Causal std     & 0.064    & 0.117    & 0.196 & 0.084       & 0.178    & 0.056    & 0.121\\
       \hline
       Causal rel err & 2.984   & 8.689    & 24.859 & 1.182       & 31.605   & 8.367    & 6.296\\
       \hline
    \end{tabular}
    \caption{Results comparing best mean squared error $\mathbb{E}[(Y - h)^2]$. Model used: eq(89)-eq(94), standardised. RKHS hyperparameter used: $al$= median interpoint distance, 1.655, $bl= 94.44$, sem name: rbfNonLinearYFullTrain10000scaledSig2. Training size: 7000 \textcolor{red}{details are for our own record, remove for submission.}
}
    \label{tab:mse}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Models & MMR(rkhs)& MMR(NN) & NN-regression & NN2SLS\\
       \hline
       Full Graph & - & - & - & - \\
       \hline
       Simple Graph & - & - & - & -\\
       \hline
    \end{tabular}
    \caption{Results comparing best mean squared error $\mathbb{E}[(\mathbb{E}[Y|A,X,Z] - \mathbb{E}[h|A,X,Z])^2]$}
    \label{tab:mse}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Models & MMR(rkhs)& MMR(NN) & NN-regression & NN2SLS\\
       \hline
       Full Graph & 4.41 & - & - & - \\
       \hline
       Simple Graph & 2.1 & 3.09 & - & -\\
       \hline
    \end{tabular}
    \caption{Results comparing best mean absolute error on ATE}
    \label{tab:mae}
\end{table}

We also show the visualisations of $h$ to further illustrate the validity of our results.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.5]{plots/MMR_plots/asinaMild/h_trainsz3000_seed8.png}
    \caption{Visualisation of h given by MMR(rkhs)}
    \label{fig:h} %  with sigma=8.458585549605719, delta = 90, but since this is only for illustrative purpose, the exact hparam probs doesn't matter much.
\end{figure}
